Modeling Multiple Irregularly Spaced Financial Time Series

In this paper we propose univariate volatility models for irregularly spaced financial time series by modifying the regularly spaced stochastic volatility models. We also extend this approach to propose multivariate stochastic volatility (MSV) models for multiple irregularly spaced time series by modifying the MSV model that was used with daily data. We use these proposed models for modeling intraday logarithmic returns from health sector stocks data obtained from Trade and Quotes (TAQ) database at Wharton Research Data Services (WRDS).

==> plan.tex <==
\iffalse
\section{Plan}

\begin{itemize}
    \item \textbf{Use of Logarithmic vector multiplicative error model specification of \cite{taylor2017logarithmic} with multivariate gamma errors. (Call it $\text{Log-vMEM}_{1}$)}.
    \item \textbf{Propose another Logarithmic vector multiplicative error model specification by generalizing the $\text{Log-ACD}_{2}$ model of \cite{bauwens2000logarithmic} with multivariate Gamma errors. (Call it $\text{Log-vMEM}_{2}$)}.
    \item \textbf{Derive the stationarity conditions of $\text{Log-vMEM}_{1}$ and $\text{Log-vMEM}_{2}$ model.}
    \item \textbf{Introduce structured regularization structures as in \cite{nicholson2020high}}
    \item \textbf{Penalized Likelihood Inference and its estimation using Coordinate Descent Approach}
    \item \textbf{Simulation}
    \item \textbf{Empirical Results}
          \begin{itemize}
                \item Let $\boldsymbol{x}_t =(\sqrt{RV}_t, BPV_t,RR_t,RK_t,|r_t|)'$ be a 5-dimensional time series each of length T.
                \item  Forecast realized volatility measures for liquid and illiquid stocks of NYSE 
          \end{itemize}
    \item \textbf{Discussion and Conclusion}
\end{itemize}
